Automatic feature learning for vulnerability prediction

Code flaws or vulnerabilities are prevalent in software systems and can potentially cause a variety of problems including deadlock, information loss, or system failure. A variety of approaches have been developed to try and detect the most likely locations of such code vulnerabilities in large code bases. Most of them rely on manually designing features (e.g. complexity metrics or frequencies of code tokens) that represent the characteristics of the code. However, all suffer from challenges in sufficiently capturing both semantic and syntactic representation of source code, an important capability for building accurate prediction models. In this paper, we describe a new approach, built upon the powerful deep learning Long Short Term Memory model, to automatically learn both semantic and syntactic features in code. Our evaluation on 18 Android applications demonstrates that the prediction power obtained from our learned features is equal or even superior to what is achieved by state of the art vulnerability prediction models: 3%--58% improvement for within-project prediction and 85% for cross-project prediction.

==> sections/discussion.tex <==
\section{Discussion}

The promising results from our evaluation suggest that a good language model for software code can be built based on the powerful, deep learning-based LSTM architecture. Our next step involves conducting an extrinsic evaluation to measure the performance of our language model at a number of real SE tasks. For example, we will develop our language model into a \emph{code suggestion} engine. This engine will suggest a sequence of code tokens that fit most with the current context and is most likely to appear next. %The code at the current position and the suggested sequence together form a meaningful piece of code.

Our language model can also provide us with a deep, semantic representation for any arbitrary sequence of code tokens. This can be done by aggregating all the output vectors ($h_{1}$, ..., $h_k$) through a mechanism known as pooling. The simplest method is mean-pooling where the vector representing a code sequence is the sum of the output vectors of all the code token in the sequence divided by the number of tokens. This representation is in the form of a feature vector, which can be readily input to any classifier to learn many useful SE tasks such as defect prediction, checking for code duplication, and detecting vulnerable software components. As we have seen, this feature vector is learned automatically (in an unsupervised manner) from the raw code, removing us from the time-consuming task of manually designing features (which have been done in previous work).

The language model for software code is part of DeepSoft -- our generic, dynamic deep learning-based framework for modeling software and its development and evolution process. DeepSoft is a compositional architecture which has several layers modeling the progression of a software at four levels: source code, issue reports, releases, and project. Each layer employs chain of LSTM units  to capture the sequential nature of the corresponding data. We envision many applications of DeepSoft to SE problems ranging from requirements to maintenance such as risk prediction, effort estimation, issue resolution recommendation, code patch generation, release planning, and developer modeling.


%DeepSoft is a compositional architecture in which an output from a module (e.g. an LSTM unit) can be used as input for the next module (another LSTM unit in the same or different layer), making it a deep architecture.

%For example, a each vector representation for each issue report is developed in a similar manner (i.e. automatically learned) to how we built for source code here. The issue vectors are aggregated to form a vector representation for the issue. The issue vector is also matched with the vector of its associated code patch. All of these combinations make DeepSoft a very powerful, deep architecture that support many software engineering tasks such as issue resolution recommendation, code patch generation, release planning, and developer modeling.



==> sections/old/approach.tex <==
\section{Approach}

\begin{figure*}[ht]
	\centering
	\includegraphics[width=\linewidth]{figs/LSTM-BoW}
	\caption{A deep model for predicting code vunerability}
	\label{fig:LSTM-CLB}
\end{figure*}

\subsection{Overview}

%\todo{SUGGEST ADD NUMBERS TO THE FIGURE 4 e.g. (1), (2) etc and refer to these in the text below?}

The process of learning function $vuln(x)$ for software vulnerability
detection goes through multiple processes (see Figure \ref{fig:LSTM-CLB}).
We consider each Java source file as consisting of a header (which
contains a declaration of class variables) and a set of methods. We
treat a header as a special method (method 0). We parse the code within
each method into a \emph{sequence of code tokens}, which is fed into
into a Long Short-Term Memory (LSTM) system to learn a vector representation
of the method (i.e. \emph{method features}). This important step transforms
a variable-size sequence of code tokens into a fixed-size feature
vector in a multi-dimensional space.

After this process, we obtain a set of feature vectors, one for each
method in a file. The next step is aggregating those feature vectors
into a single feature vector. The aggregation operation is known as
\emph{pooling}. The simplest method is mean-pooling where we take
the sum of the method vectors and divide it by the number of methods
in a file. More complex pooling methods can be used and we will discuss
it in more details. This process produces a set of features for a
file (i.e. \emph{LSTM features}).

Each source file is tokenized into a vector of code tokens and the
frequency of each token in the file is counted. Those term frequencies
are used to produce another set of features for a file (i.e. \emph{BoW
features}). We combine both LSTM and BoW features and fed them to
a classifier. This classifier is trained and used for predicting vulnerability.
We now describe each of these processes in details.

\subsection{Parsing source code \label{subsec:Parsing-source-code}}

We use Java Abstract Syntax Tree (AST) to extract syntactic information
from source code. To do so, we utilize JavaParser\footnote{\url{http://javaparser.org}}
to lexically analyze each source file and obtain an AST. Each source
file is parsed into a set of methods and each method is parsed into
a sequence of code tokens. All class attributes (i.e. the header)
are grouped into a sequence of tokens. Comments and blank lines are
ignored. Following standard practice (e.g. as done in \cite{White:2015:TDL}),
we replace integers, real numbers, exponential notation, and hexadecimal
numbers with a generic $\langle num\rangle$ token, and replace constant
strings with a generic $\langle str\rangle$ token. We also replace
less popular tokens (e.g. occurring only once in the corpus) and tokens
which exist in test sets but do not exist in the training set with
a special token $\langle unk\rangle$. A fixed-size vocabulary $\mathscr{V}$
is constructed based on top $N$ popular tokens, and rare tokens are
assigned to $\langle unk\rangle$. Doing this makes our corpus compact
but still provides partial semantic information.

%\todo{WHY IS THE ABOVE DONE - the replacements - EXPLAIN BRIEFLY e.g. not to confuse the learner?}
%Finally, we build a code corpus of 6,103,191 code tokens, with a vocabulary of 81,213 \emph{unique} tokens.

%Each sequence is then split into sentences (i.e a subsequence of code tokens) of fixed length. We use 10K sentences for each case of training, validation and testing. Sentence length varies from 10 (e.g., a short statement), to 500 (e.g., a large file). Embedding dimensionality ($D$) varies from 20 to 500. For simplicity, the size of the memory (i.e. the size of $\cb_{t}$) is the same as the number of embedding dimensions, that is $D=K$.

\subsection{Method features \label{subsec:Method-features}}

%\todo{I wondered if a sentence or two on why doing this conversion would help a non-ML / non-DL reader???}

After the parsing and tokenizing process, each method is now a sequence
of code tokens $\langle w_{1},w_{2},...,w_{n}\rangle$. We then use
LSTM to automatically learn features from the code sequence in a method
(see Figure \ref{fig:LSTM-example-1}). An LSTM unit takes as input
a vector representing a code token. Hence, we need to convert each
code token into a fixed-length continuous vector. This process is
known as \emph{code token embedding}. We do so by maintaining a token
embedding matrix $\mathcal{M}\in\mathbb{R}^{d\times|\mathscr{V}|}$
where $d$ is the size of a code token vector and $|\mathscr{V}|$
is the size of vocabulary $\mathscr{V}$. Each code token has an index
in the vocabulary, and this embedding matrix acts as a look-up table:
each column $i^{th}$ in the embedding matrix is an embedded vector
for the token $i^{th}$. We denote $\xb_{t}$ as a vector representation
of code token $w_{t}$. For example, token ``try'' is converted
in vector {[}0.1, 0.3, -0.2{]} in the example in Figure \ref{fig:LSTM-example-1}.

\begin{figure}[ht]
\centering \includegraphics[width=1\linewidth]{figs/LSTM-example-1}
\caption{An example of how a vector representation is obtained for a code sequence}
\label{fig:LSTM-example-1}
\end{figure}

The code sequence vectors that make up each method are then input
to a sequence of LSTM units. Specifically, each token vector $\xb_{t}$
in a sequence $\langle\xb_{1},\xb_{2},...,\xb_{n}\rangle$ is input
into an LSTM unit (see Figure \ref{fig:LSTM-example-1}). All the
LSTM units share the same model parameters which are denoted as a
weight matrix $\mathcal{U}\in\mathbb{R}^{d'\times|\mathscr{V}|}$.
This embedding matrix $\mathcal{U}$ is used to compute the output
state $\Sb_{t}$ for an input token $\xb_{t}$. For example in Figure
\ref{fig:LSTM-example-1}, the output state vector for code token
``try'' is {[}0.1, 0.3, -0.2{]}. The size of this vector can be
different from the size of the input token vector (i.e. $d\neq d'$),
but for simplicity in training the model we assume they are the same.

% : column $k^{th}$ in matrix $\mathcal{U}$ returns a vector for a word having index $k$ in the vocabulary

%Note that matrix $\mathcal{U}$ also acts as a look-up table for each word in the vocabulary \mathscr{V}, i.e. the number of columns in matrix $\mathcal{U}$ is equal to the size of the vocabulary $|\mathscr{V}|$.

%\subsection{Training}

%\todo{for the non-ML expert - why doing this - sentence or two e.g. "We then need to train the LTSM in order to ...}
% The advantage of this training is that it can be done \emph{without} using vulnerability labels
LSTM automatically learns both model parameters $\mathcal{U}$ and
the code token embedding matrix $\mathcal{M}$ by predicting the next
code token. Specifically, we use the output state vector of code token
$w_{t}$ to predict the next code token $w_{t+1}$ from a context
of earlier code tokens $\wb_{1:t}$ by computing a posterior distribution:

\begin{equation}
P\left(w_{t+1}=k\mid\wb_{1:t}\right)=\frac{\exp\left(\mathcal{U}_{k}^{\top}\Sb_{t}\right)}{\sum\limits _{k'}\exp\left(\mathcal{U}_{k}^{\top}\Sb_{t}\right)}\label{eq:softmax}
\end{equation}
where $k$ is the index of token $w_{t+1}$ in the vocabulary, $\mathcal{U}^{\top}$
the transpose of matrix $\mathcal{U}$, and $\mathcal{U}_{k}^{\top}$
indicates the vector in column $k^{th}$ of $\mathcal{U}^{\top}$,
and $k'$ runs through all the indices in the vocabulary, i.e. $k'\in\{1,2,...,|\mathscr{V}|\}$.
This learning style essentially estimates a language model of code,
as evidenced by the chain-rule:
\begin{equation}
P\left(w_{1},w_{2},...,w_{n}\right)=P(w_{1})\prod_{t=1}^{n-1}P\left(w_{t+1}\mid\wb_{1:t}\right)\label{eq:lang-model}
\end{equation}
Thus the LSTM automatically learns a grammar of code \cite{giles2001noisy}.

\subsubsection{Model training}

LSTM can automatically train itself using code sequences in all the methods extracted from our dataset. During training, for every token in a sequence $\langle w_{1},w_{2},...,w_{n}\rangle$, we know the true next token. For example, the true next token after
``try'' is ``\{'' in the example Figure \ref{fig:LSTM-example-1}.
We use this information to learn the model parameters which maximize
the accuracy of our next token predictions. To measure the accuracy,
we use the log-loss (i.e. the cross entropy) of each true next token,
i.e. $-\log P(w_{1})$ for token $w_{1}$, $-\log P(w_{2}\mid w_{1}$)
for token $w_{2}$, ..., $-\log P\left(w_{n}\mid w_{1:n-1}\right)$
for token $w_{n}$. The model is then trained using many known sequences
of code tokens in a dataset by minimizing the following sum log-loss
in each sequence:

\begin{equation}
L(\mathcal{U})=-\log P(w_{1})-\sum_{t=1}^{n-1}\log P\left(w_{t+1}\mid\wb_{1:t}\right)\label{eq:log-loss}
\end{equation}
which is essentially $-\log P\left(w_{1},w_{2},...,w_{n}\right)$.

%\todo{need to explain what "pooling" is and why this formula chosen?}

Learning involves computing the gradient of $L(\mathcal{U})$ during
the back propagation phase, and the model parameters $\mathcal{U}$
are updated using a stochastic gradient descent.

\subsubsection{Method feature extraction}

Once the training phase has been completed we use the learned model
parameter $\mathcal{U}$ to compute a output state vector $\Sb_{t}$
for every code token $\wb_{t}$ in an input sequence. We then compute
a vector $\bar{\Sb}$ for the method by aggregating all the vector
states (see Figure \ref{fig:LSTM-example-1}) so that all information
from the start to the end of a method is accumulated. This process
is known as \emph{pooling} and there are multiple ways to perform
pooling, but the main requirement is that pooling must be length invariant,
that is, pooling is not sensitive to variable method lengths. We employ
a simple but often effective pooling method, which consists of (a)
mean pooling, i.e. $\bar{\Sb}=\frac{1}{n}\sum\limits _{t=1}^{n}\Sb_{t}$,
and (b) variance pooling, i.e., $\sigmab=\sqrt{\frac{1}{n}\sum\limits _{t=1}^{n}\left(\Sb_{t}-\bar{\Sb}\right)\ast\left(\Sb_{t}-\bar{\Sb}\right)}$
, where $\ast$ denotes element-wise multiplication. Thus, a method
is represented by a concatenated feature vector $\qb=\left[\bar{\Sb},\sigmab\right]$.

\subsection{LSTM file features}

% the next problem to tackle is the ability to string words together appropriately in small, grammatically correct sentences which make sense.

The previous step generates a vector of features representing each
method in a file. We need to aggregate all method features to a single
set of features representing a file. This again can be done through
another pooling mechanism, which aims to transform the joint feature representation (e.g. method features) into a new, more usable one (e.g. file features) that maintain
important information while removing irrelevant detail.  We consider two kinds of pooling: one is based on statistics over the set of method vectors, and the other is based on building a codebook.

\subsubsection{Statistical features}

For this pooling method, we use simple statistics over set of method
vectors, similar to those used in pooling token states into method
vectors. In particular, given a file as a collection of methods, each
of which is represented as a vector, we collect element-wise statistics
including \emph{mean}, \emph{standard deviation}, \emph{min} and \emph{max}.
All of those statistics are then concatenated into a single vector
representing the file.

\subsubsection{Codebook}

Borrowing the concept from the computer vision community, we consider
each method in a file as an analogy for a salient point (i.e., the
most informative point) in an image. The method vector representation
is akin to the set of point descriptors such as SIFT \cite{lowe1999object}.
The main difference here is that in vision, visual descriptors are
calculated manually, whereas in our setting, method representation
is learnt automatically. In vision, descriptors are clustered into
a set of points called a \emph{codebook} (not to be confused with
the software source code), which is essentially the descriptor centroids.


\begin{figure}[ht]
\centering \includegraphics[width=1\linewidth]{figs/codebook-methods}
\caption{An example of using ``codebook'' to automatically learn file features from method features}
\label{fig:codebook}
\end{figure}

Likewise we can also build a codebook that summarizes all software
methods. Each ``code'' in the codebook represents a distinct region
\emph{in the semantic space of methods}. We construct a codebook by using $k$-means to cluster all method vectors in the training set, where $k$ is the pre-defined number of centroids, and hence the size of the codebook (see Part A in Figure \ref{fig:codebook}, each small circle representing a method vector in the space). The example in Figure \ref{fig:codebook} uses $k=3$ to produce three method clusters. For each new file, we obtain all the method vectors (Part B in Figure \ref{fig:codebook}) and assign each of them to the closest centroids (Part C in Figure \ref{fig:codebook}). The file is represented as a vector of length $k$, whose elements are the number of centroid occurrences. For example, the new file in Figure \ref{fig:codebook} has 10 method vectors. We then compute the distances between those vectors to the three centroids established in the training set. We find that 3 of them are closest to centroid \#1, 2 to centroid \#2 and 5 to centroid \#3. Hence, the feature vector for the new file would be [3, 2, 5].

This technique provides a powerful abstraction over a number of methods in a file. The intuition here is that the number of methods in an entire dataset could be large but the number of method types (i.e. the method clusters) can be small. Hence, an file can be characterized by the types of the methods it contains. This approach offers an efficient and effective way to learn new features for a file from its methods. In effect, a file is a collection of distinct regions in the semantic space of methods.

%It can also be used in combination with the statistical aggregation approach to provide an in-depth set of features for an iteration.

\subsection{BoW file features}

LSTM learns the grammars, that is, the set of hidden rules for code tokens to work with each other. Since we trained LSTM to predict the next tokens (i.e. code completion), information from previous tokens must be predictive or the next tokens. Hence, our LSTM features captures the syntactical structures in in each method in a source file. Our approach also makes use of features extracted from the Bag-of-Words (BoW) approach to capture the lexical statistics at the file level. Previous work \cite{ScandariatoWHJ14} has demonstrated that features extracted from the BoW lexical statistics are highly robust in vulnerability prediction. Hence, our approach combine both LSTM features and BoW features into a single set of features representing a file.

The BoW features are automatically extracted as follow. After the tokenizing process, we count the frequency of each token in the file. Previous work \cite{ScandariatoWHJ14} has found that the discretization of the BoW features significantly improves the performance of the vulnerability prediction models. Thus, we also adopted this approach by transforming the numerical BoW features into two \emph{bins}. If a code token occurs more than a certain threshold (e.g. 5 times) than it is mapped to one bin, otherwise it is mapped to another bin.

\subsection{Vulnerability prediction}


Using the process above, we generate the features for each file in both the training data and the test data. We then use the standard process described in Section \ref{sect:vuln-prediction} to build and train vulnerability prediction models. Files in the test data are used to assess the performance of the trained prediction models.

%\todo{I think it would be nice to complete this section with a brief explanation of what we now have - a tool that can take a set of Java files ; turn them into vectors ; train a RNN using a bunch of benchmark Java projects to recognise vulnerabilities within method and between methods ; and when given a Java project, predict likely areas of vulnerability - at method level or only file level????}

%\todo{I didn't quite get how the training works - what is the input - set of Java projects - but HOW recognise the vulnerable areas in code - how are these indicated to the trainer??? }

%\paragraph{Remarks}

%We emphasize here is that the feature extraction is entirely unsupervised,
%that is, no label is used.



==> sections/old/background.tex <==
\section{Background}


\subsection{Vulnerability prediction}\label{sect:vuln-prediction}

Vulnerability prediction typically involves determining whether a source code file is likely to be vulnerable. The goal is to alert software engineers with parts of the code base that deserve particular attention, rather than pinpointing exactly the code line where a vulnerability is resided. Hence, we also choose to work at the level of files since this is also the scope of existing work (e.g. \cite{ScandariatoWHJ14,Shin:2011:ECC}) which we would like to compare our approach against.

Determining if a source file is vulnerable can be considered as a function $vuln(x)$ which takes as input a file $x$ and returns a boolean value: $true$ indicates that the file is vulnerable, while $false$ indicates that the file is clean. Vulnerability prediction is therefore to approximate this classification function $vuln(x)$ by learning from a number of examples (i.e. files known to be vulnerable or clean) provided in a \emph{training set}. After training, the learned function is used to automatically determine the vulnerability of new source files.

Machine learning techniques have been widely used to learn function $vuln(x)$. To make it mathematically and computationally convenient for machine learning algorithms, file $x$ needs to be represented as a n-dimensional vector where each dimension represents a feature (or predictor). Many existing approaches use software metrics (e.g. the number of code lines and cyclomatic complexity) to form a file's feature vector. Recent approaches use classical text mining techniques like Bag-of-Words to represent a file as a vector of term frequencies where each term is a code token.

%\subsection{Feedforward neural networks}

%The goal of a feedforward neural network is to approximate some functions such as $vuln(x)$. A feedforward network defines a mapping $y = vuln^*(x, \theta)$, and learns the value of parameters $\theta$ that leads to the best function approximation. In a feedforward network, information flows from input $x$ through a number of (hidden) layers, and finally to the output $y$. Each layer $\hb_{l}$ takes as input the output from the previous layer $\hb_{l-1}$, performs a simple transformation as below, and outputs to the next layer:

%\[
%\hb_{l}=\sigma\left(W_{l}\hb_{l-1}+\bb_{l}\right)
%\]
%where $\sigma$ is an element-wise non-linear transformation, and $\thetab_{l}=\left(W_{l},\bb_{l}\right)$ are parameters, the bottom layer is the input, i.e.  $\hb_{0}= x$, and the top layer is the output, i.e. $y=W_{L}\hb_{L}+\bb_{L}$.

%In our paper, we choose $\sigma$ to be rectifier linear unit (ReLU), that is $\sigma(x)=\max(0,x)$.

\subsection{Recurrent Neural Network and Long Short Term Memory}

A Recurrent Neural Network (RNN) \cite{hochreiter2001gradient} is a single-hidden-layer neural network repeated multiple times. While a feedforward neural network maps an input vector into an output vector, an RNN maps \textbf{a sequence into a sequence} (see Figure \ref{fig:RNN-LSTM}). Let $\wb_{1},...,\wb_{n}$ be the input sequence (e.g. code tokens) and $\yb_{1},...,\yb_{n}$ be the sequence of corresponding labels (e.g. the next code tokens). At each step $t$, a standard RNN model reads the input $\wb_{t}$ and the previous output state $\Sb_{t-1}$ to compute the output state $\Sb_{t}$ as follows.

\begin{equation}\label{eq:hidden-state}
\Sb_{t}=\sigma\left(\bb+W_{tran}\Sb_{t-1}+W_{in}\wb_{t}\right)
\end{equation}
where $\sigma$ is a nonlinear element-wise transform function, and $\bb$, $W_{tran}$ and $W_{in}$
are referred to as \emph{model parameters}. The output state is used to predict the output (e.g. the next code token based on the previous ones) at each step $t$.

% would be a vector of probabilities across our vocabulary, i.e. $softmax(V\hb_{t})$.

\begin{figure}[ht]
	\centering
	\includegraphics[width=\linewidth]{figs/LSTM-example}
	\caption{A recurrent neural network}
	\label{fig:RNN-LSTM}
\end{figure}

An RNN shares the same parameters across all steps since the same task is performed at each step, just with different inputs. Hence, using an RNN significantly reduces the total number of model parameters which we need to learn. The RNN model is trained using many input sequences with known true output sequences. The errors between the true outputs and the predicted outputs are passed backwards through the network during training to adjust the model parameters such that the errors are minimized.

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.5\linewidth]{figs/LSTMcell}
	\caption{The internal structure of an LSTM unit}
	\label{fig:LSTMunit}
\end{figure}

A Long Short-Term Memory (LSTM) \cite{hochreiter1997long,gers2000learning} architecture is a special variant of RNN, which is capable of learning long-term dependencies. Due to space limitations, we briefly describe LSTM here and refer the readers to the seminal paper \cite{hochreiter1997long} for more details. It has a \emph{memory cell} $c_t$ which stores accumulated memory of the context. The amount of information flowing through the memory cell is controlled by three gates (an \emph{input gate} $i_t$, a \emph{forget gate} $f_t$, and an \emph{output gate} $o_t$), each of which returns a value between 0 (i.e. complete blockage) and 1 (full passing through). First, an LSTM unit decides how much information from the memory of previous context  (i.e. $c_{t-1}$) should be kept in the current memory cell. This is controlled by the forget gate $\fb_{t}$, which looks at the the previous output state $s_{t-1}$ and the current code token $w_t$, and outputs a number between 0 and 1. A value of 1 indicates that all the past memory is preserved, while a value of 0 means ``completely forget everything''. For example, when processing line 1 of the code Listing 2 in Figure \ref{fig:example}, the memory cell might keep information about a lock which has been acquired. When it sees the lock released (line 9), it would remove this locking information from the memory.

The next step is updating the memory with new information obtained from the current code token $w_t$. In a similar manner to the forget gate, the input gate $\ib_{t}$ is used to control which new information will be stored in the memory. For example, if $w_t$ is ``try'', we want to add it into the memory cell so that we remember ``catching'' it later. Finally, information stored in the memory cell will be used to produce an output $h_t$. The output gate $\ob_t$ looks at the current code token $w_t$ and the previous hidden state $h_{t-1}$, and determines which parts of the memory should be output. For example, since it just saw the token ``.'', it might want to output information relevant (e.g. methods) to the object preceding this token, in case that what is coming next.

All those gates are \emph{learnable}, i.e. being trained with the whole code corpus. It is important to note here that LSTM computes the output state based on not just only the current input $w_t$ and the previous ouput state $h_{t-1}$ (as done in standard RNNs) but also the current memory cell state $c_t$, which is \emph{linear} with the previous memory $c_{t-1}$. This is the key feature allowing an LSTM model to learn long-term dependencies.


%The most important element of LSTM is a short-term \emph{memory cell} -- a vector that stores accumulated information over time. The information stored in the memory is refreshed at each time step through partially forgetting old, irrelevant information (controlled by a \emph{forget gate}) and accepting fresh new input. However, only some parts of the input will be added to the memory through a selective \emph{input gate}. Once the memory has been refreshed, an output state will be read from the memory through an \emph{output gate}. The reading of the new input, writing of the output, and the forgetting are all \emph{learnable}. LSTM has demonstrated ground-breaking results in many applications such as language models \cite{sundermeyer2012lstm}, speech recognition \cite{graves2013speech} and video analysis \cite{yue2015beyond}.


%Let us now explain how an LSTM unit works. First, an LSTM unit decides how much information from the memory of previous context  (i.e. $c_{t-1}$) should be removed from the memory cell. This is controlled by the forget gate $\fb_{t}$, which looks at the the previous output state $h_{t-1}$ and the current code token $w_t$, and outputs a number between 0 and 1. A value of 1 indicates that all the past memory is preserved, while a value of 0 means ``completely forget everything''. In our example with the description of \texttt{XD-2970} in Figure \ref{figure:example-story-point}, the memory cell might include the information that both \emph{log4j} and \emph{logback} are back-end logging libraries.

%The next step is updating the memory with new information obtained from the current code token $w_t$. In a similar manner to the forget gate, the input gate $\ib_{t}$ is used to control which new information will be stored in the memory. In our example, we would want to add \emph{logback} as an alternative back-end logging library to the memory cell. Finally, information stored in the memory cell will be used to produce an output $h_t$. The output gate $\ob_t$ looks at the current code token $w_t$ and the previous hidden state $h_{t-1}$, and determines which parts of the memory should be output. For example, since we just saw ``\emph{replace log4j with}'', we would output an alternative back-end logging library, in case that what is coming next.





%Learning involves computing the gradient of $L(\thetab)$ during the backpropagation phase, and parameters are updated using a stochastic gradient descent (SGD). It means that parameters are updated after seeing only a small random subset of sequences.


%The critical problem with standard RNNs however lies here where the magnitude of weights in the transition matrix $W_{tran}$ (used in Equation~\ref{eq:hidden-state}) can have a strong effect on the learning process. This is because during the gradient backpropagation phase, the gradient signal can be multiplied a large number of times (as many as the number of code tokens in a sequence) by the transition matrix. If the weights in this matrix are small, it can result in the problem of \emph{vanishing gradients} where the gradient signal becomes so small that the learning gets very slow or even stopped. This makes standard RNNs not suitable for learning long-term dependencies. On the other hand, the large weights can lead to a large gradient signal (e.g. \emph{exploding gradient}), which can cause learning to diverge.


%\subsection{Long Short-Term Memory}

%The inherent vanishing or exploding gradients issue in RNNs make them very hard to train for long sequences \cite{bengio2013advances}. Consider trying to predict the last word in the following text extracted from the description of issue \texttt{XD-2970} in Figure \ref{figure:example-story-point}: \emph{``Boot uses slf4j APIs backed by logback. This causes some build incompatibilities .... An additional step is to replace log4j with \underline{\space\space\space\space}.''}. Recent information suggests that the next word is probably the name of a logging library, but if we want to narrow down to a specific library, we need the context of \emph{logback} as an alternative back-end logging library, from further back. There could be a big gap between relevant information and the point where it is needed. Unfortunately, as that gap increases, RNNs will not be able to learn to connect the information.


==> sections/old/conclusions.tex <==
\section{Conclusions and future work}

Conclusions and future work goes here.

Different types of applications and programming languages

Finer grained granularity, e.g. code changes, methods. 

Expand to defect prediction. 


==> sections/old/discussion.tex <==
\section{Discussion}

The promising results from our evaluation suggest that a good language model for software code can be built based on the powerful, deep learning-based LSTM architecture. Our next step involves conducting an extrinsic evaluation to measure the performance of our language model at a number of real SE tasks. For example, we will develop our language model into a \emph{code suggestion} engine. This engine will suggest a sequence of code tokens that fit most with the current context and is most likely to appear next. %The code at the current position and the suggested sequence together form a meaningful piece of code.

Our language model can also provide us with a deep, semantic representation for any arbitrary sequence of code tokens. This can be done by aggregating all the output vectors ($h_{1}$, ..., $h_k$) through a mechanism known as pooling. The simplest method is mean-pooling where the vector representing a code sequence is the sum of the output vectors of all the code token in the sequence divided by the number of tokens. This representation is in the form of a feature vector, which can be readily input to any classifier to learn many useful SE tasks such as defect prediction, checking for code duplication, and detecting vulnerable software components. As we have seen, this feature vector is learned automatically (in an unsupervised manner) from the raw code, removing us from the time-consuming task of manually designing features (which have been done in previous work).

The language model for software code is part of DeepSoft -- our generic, dynamic deep learning-based framework for modeling software and its development and evolution process. DeepSoft is a compositional architecture which has several layers modeling the progression of a software at four levels: source code, issue reports, releases, and project. Each layer employs chain of LSTM units  to capture the sequential nature of the corresponding data. We envision many applications of DeepSoft to SE problems ranging from requirements to maintenance such as risk prediction, effort estimation, issue resolution recommendation, code patch generation, release planning, and developer modeling.


%DeepSoft is a compositional architecture in which an output from a module (e.g. an LSTM unit) can be used as input for the next module (another LSTM unit in the same or different layer), making it a deep architecture.

%For example, a each vector representation for each issue report is developed in a similar manner (i.e. automatically learned) to how we built for source code here. The issue vectors are aggregated to form a vector representation for the issue. The issue vector is also matched with the vector of its associated code patch. All of these combinations make DeepSoft a very powerful, deep architecture that support many software engineering tasks such as issue resolution recommendation, code patch generation, release planning, and developer modeling.



==> sections/old/evaluation.tex <==
\section{Evaluation}

We describe an evaluation of our new technique for Java code vulnerability prediction using a large dataset used in previous prediction work, and compare the performance of our approach to two previous techniques.

\subsection{Datasets}

To carry out our empirical evaluation, we exploited a publicly available dataset \cite{Scandariato2014Dataset} that has been used in previous work \cite{ScandariatoWHJ14} for vulnerability prediction. This dataset originally contained 20 popular applications which were collected from F-Droid and Android OS in 2011. The dataset covers a diversity of application domains such as education, book, finance, email, images and games. However, the provided dataset only contained the application names, their versions (and dates), and the file names and their vulnerability labels. It did not have the source code for the files, which is needed for our study. Using the provided file names and version numbers, we then retrieved the relevant source files from the code repository of each application.


\begin{table}[h]
	\centering
	\caption{Dataset statistics}
	\label{table:dataset-stats}
	\resizebox{3.5in}{!}{%
		\begin{tabular}{@{}lcccccc@{}}
			\toprule
			%\multicolumn{1}{c}{\multirow{2}{*}{Project}} & \multicolumn{3}{c}{Training set} & \multicolumn{3}{c}{Test set} \\ \cmidrule(l){2-4}\cmidrule(l){5-7}
			App         & \#Versions     & \#Files    & Mean files       & Mean LOC   & Mean Vuln   & \% Vuln    \\
			\midrule
            Crosswords & 16 & 842 & 52 &  12,138 & 24 & 0.46 \\
            Contacts&6&787&131&39,492&40&0.31 \\
            Browser&6&433&72&23,615&27&0.37 \\
            Deskclock&6&127&21&4,384&10&0.47 \\
            Calendar&6&307&51&21,605&22&0.44 \\
            AnkiAndroid&6&275&45&21,234&27&0.59 \\
            Mms&6&865&144&35,988&54&0.37 \\
            Boardgamegeek&1&46&46&8,800&11&0.24 \\
            Gallery2&2&545&272&68,445&75&0.28 \\
            Connectbot&2&104&52&14,456&24&0.46 \\
            Quicksearchbox&5&605&121&15,580&26&0.22 \\
            Coolreader&12&423&35&14,708&17&0.49 \\
            Mustard&11&955&86&14,657&41&0.47 \\
            K9&19&2,660&140&50,447&65&0.47 \\
            Camera&6&457&76&16,337&29&0.38 \\
            Fbreader&13&3,450&265&32,545&78&0.30 \\
            Email&6&840&140&51,449&75&0.54 \\
            Keepassdroid&12&1,580&131&14,827&51&0.39 \\
			 \bottomrule
		\end{tabular}
	}
\end{table}

We could not find the code repository for two applications since they appeared no longer available. For some apps, the number of versions we could retrieve from the code repository is less than that in the original datasets. For example, we retrieve the source files for 16 versions of Crossword while the original dataset had 17 versions. The source files for some older versions were no longer maintained in the code repository. Table \ref{table:dataset-stats} provides some descriptive statistics for 18 apps in our dataset, including the number of versions, the total number of files, the average number of files in a version, the average number of lines of code in a version, the average number of vulnerable files in a version, and the ratio of vulnerable files.

\subsection{Research questions}

Our evaluation focuses on comparing our model against other state-of-the-art techniques in vulnerability prediction. To facilitate this comparison, we followed previous work \cite{ScandariatoWHJ14} and aimed to answer the following research questions .

      \begin{itemize}
        \item \textbf{RQ1. Within-project prediction}: \emph{Are the automatically learned features using LSTM suitable for building a vulnerability prediction model?}

        To answer this question, we focused on one version (the first one) in each application in our dataset. We ran a cross-fold validation experiments by dividing the files in each application into 10 folds, each of which have the approximately same ratio between vulnerable files and clean files. Each fold is used as the test set and the remaining folds are used for training. As a result, we built 10 different prediction models and the performance indicators are averaged out of the 10 folds.


        \item \textbf{RQ2. Cross-version prediction}: \emph{How does our proposed approach perform in predicting future releases, i.e. when the model is trained using an older version in application and tested on a newer version in the same application?}

        In this second experiment, all the files in the first version of each application are used to train a prediction model, which is then used to predict vulnerability of the files of all subsequent versions. For example, the first version in the Crosswords app is used to training and each of the remaining 15 versions is used as a test set.

        \item \textbf{RQ3. Cross-project prediction}:\emph{ Is our approach suitable for cross-project predictions where the model is trained using a source application and tested on a different application?}

            In the third experiment, we used all the files in the first version of each project for training a prediction model. This model is then tested on the first version of the remaining applications.

      \end{itemize}


\subsection{Benchmarks}

We compare the performance of our approach against two techniques that have been widely used for predicting vulnerabilities in code.

\textbf{Software metrics}:  Complexity metrics have been extensively used for defect prediction (e.g. \cite{Hall:2012}) and vulnerability prediction (e.g. \cite{Shin:2011:ECC,Shin:2008:EMP,Chowdhury:2011:UCC}). This is resulted from the intuition that complex code is difficult to understand, maintain and test, and thus has a higher chance of having vulnerabilities than simple code. We have implemented a vulnerability prediction models based on 60 metrics. These features are commonly used in existing vulnerability prediction models. They covers 7 categories:  cohesion metrics (i.e. measure to what extent the source code elements are coherent in the system), complexity metrics (i.e. measure the complexity of source code elements such as algorithms), coupling metrics (i.e. measure the amount of interdependencies of source code elements), documentation metrics (i.e. measure the amount of comments and documentation of source code elements), inheritance metrics (i.e. measure the different aspects of the inheritance hierarchy), code duplication metrics (i.e.), and size metrics (e.g. number of code lines, and number of classes or methods).

%A number of features can be derived from complexity code metrics such as the number of lines of code in a file, the number of functions defined in a file, the number of lines of code in a file devoted to declarations, the number of lines of code in a file devoted to preprocessing, and a set of McCabe complexity metrics [5] such as the sum of essential complexity which reflects how structured a program is, the sum of strictly cyclomatic complexity where strict cyclomatic complexity is the number of conditional statements in a function, the sum of the maximum nesting level of control constructs (e.g. if or while statements) in a function, and the maximum of strict cyclomatic complexity in a file. There are also a number of metrics related to the degree of coupling between functions such as the sum of the number of inputs to a function including parameters and global variables, and the sum of the number of assignment to the parameters to call a function or global variables. Metrics regarding the level of documentation can be for example the ratio of lines of comments to line of code.

\textbf{Bag of Words}: This technique has been used in previous work \cite{ScandariatoWHJ14}, which also consider source code as a special form of text. Hence, it treats a source file as a collection of terms associated with frequencies. The term frequencies are the features which are used as the predictors for a vulnerability prediction model. Lexical analysis is done to source code to break it into a vector of code tokens and the frequency of each token in the file is counted. We also followed previous work \cite{ScandariatoWHJ14} by discretizing the BoW features since they found that this method significantly improved the performance of the vulnerability prediction models. The discretization process involves transforming the numerical BoW features into two \emph{bins}. If a code token occurs more than a certain threshold (e.g. 5 times) than it is mapped to one bin, otherwise it is mapped to another bin.


To enable a fair comparison, we use the same classifier for our prediction model and all the benchmarks. We chose Random Forests (RF), an ensemble method which combines the estimates from multiple estimators since it is one of the most effective classifier for vulnerability prediction \cite{ScandariatoWHJ14}. RF achieves a significant improvement over the decision tree approach by generating many classification and regression trees, each of which is built on a random resampling of the data, with a random subset of variables at each node split. Tree predictions are then aggregated through averaging.

\subsection{Performance measures}

%Reporting the average of precision/recall across the two classes (vulnerable and clean) is likely to overestimate the true performance, since our dataset is imbalance (i.e. the number of vulnerable files are small). More importantly, predicting vulnerable files is more of interest than predicting clean files. Hence, our evaluation is focus on the vulnerable class. 

A confusion matrix is  used to store the correct and incorrect decisions made by a prediction model. For example, if a file is classified as vulnerable when it is truly vulnerable, the classification is a true positive (tp). If the file is classified as vulnerable when it is actually clean, then the classification is a false positive (fp). If the file is classified as clean when it is in fact vulnerable, then the classification is a false negative (fn). Finally, if the issue is classified as clean and it is in fact clean, then the classification is true negative (tn). The values stored in the confusion matrix are used to compute the widely-used Precision, Recall, and F-measure for the vulnerable files to evaluate the performance of the predictive models:

\begin{itemize}
	\item{Precision:} The ratio of correctly predicted vulnerable files over all the files predicted as being vulnerable. It is calculated as: \begin{displaymath}pr=\frac{tp}{tp+fp}\end{displaymath}
	\item{Recall:} The ratio of correctly predicted vulnerable files over all of the true vulnerable files. It is calculated as: \begin{displaymath}re=\frac{tp}{tp+fn}\end{displaymath}
	\item{F-measure:} Measures the weighted harmonic mean of the precision and recall. It is calculated as: \begin{displaymath}F-measure=\frac{2*pr*re}{pr+re}\end{displaymath}
%	\item{Area Under the ROC Curve (AUC)} is used to evaluate the degree of discrimination achieved by the model. The value of AUC is ranged from 0 to 1 and random prediction has AUC of 0.5. The advantage of AUC is that it is insensitive to decision threshold like precision and recall. The higher AUC indicates a better prediction.
\end{itemize}



%The dataset however only provides the labels and the project versions but not the actual source code of these


\subsection{Model training}



\input{sections/results}


==> sections/old/implementation.tex <==
\section{Implementation}


The proposed approach is implemented in Theano\footnote{http://deeplearning.net/software/theano},
a well-respected environment for deep learning, running in Python.
It supports automatic differentiation of the loss in Eq.~(\ref{eq:log-loss})
and a host of powerful adaptive gradient descent methods. In particular
we use RMSprop as the optimizer with learning rate of 0.02, and smoothing
hyper-parameters: $\rho=0.99$, $\epsilon=1e-7$. The model parameters
are updated in a stochastic fashion, that is, after every mini-batch
of size $50$. We use $|\mathscr{V}|=5,000$ most frequent tokens
for learning the code language model in Eq.~(\ref{eq:lang-model}).
In what follows, we describe computational challenges and how to handle
them.

\subsection{Handling large vocabulary}

To evaluate the prediction probability in Eq.~(\ref{eq:softmax})
we need to iterate through all unique tokens in the vocabulary. Since
the vocab size is large, this can be very expensive. To tackle the
issue, we employ an approximate method known as Noise Contrastive
Estimation \cite{gutmann2012noise}, which allows to approximate the
vocab at each probability evaluation by a small subset of words randomly
sampled from the vocab. We use $100$ words, as it is known to work
well in practice \cite{DeepCode2016}.

\subsection{Handling long methods}

Methods are variable in size. This makes learning inefficient because
we need to handle each method separately, not making use of recent
advances in Graphical Processing Units (GPUs). A better way is to
handle methods in mini-batch of fixed size. A typical way is to pad
short methods with dummy tokens so that all methods in the same mini-batch
have the same size. However, since some methods are very long, this
approach will result in a waste of computational effort to handle
dummy tokens. Here we use a simple approach to split a long method
into non-overlapping sequences of fixed length $T$, where $T=100$
is arbitrarily chosen in this implementation. We can treat each sequence
as if it is a separate method.

\subsection{Token or sequence embedding}

After learning, each token is represented by a state vector in the
corresponding LSTM. This suggests that we can treat each file as a
collection of token vectors, inspired by success of prior work using
Bag-of-Words \cite{ScandariatoWHJ14}. However, since the number of
tokens in the training data is huge, this proves unsaleable. Thus
we use the sequence pooling described earlier in Section~\ref{subsec:Method-features}
to reduce the data.

%\begin{itemize}
%  \item The vulnerability of a method in a file can affect the vulnerability of the file. For example, if a method is vulnerable, i.e. containing some vulnerable code, then the file is also vulnerable. So we need to learn vulnerable patterns of code at the method level. Note here that we don't have vulnerability information at the method level. Multi layer network would help refine the features.
%  \item Method may interact with each other, e.g. one method calls the other. The interaction may introduce or remove vulnerability. Sharing information between columns.
%  \item Some file-level attributes (code churns, etc. in previous work) may correlate to the vulnerability outcome of the files. Taking file attributes into account.
%\end{itemize} 

==> sections/old/intro.tex <==
\section{Introduction}

%\point{Impact of cybersecurity --- cost of security bugs}

A software vulnerability -- a security flaw, glitch, or weakness found in software systems -- can potentially cause significant damages to businesses and people's lives, especially with the increasing reliance on software in all areas of our society. For instance, the Heartbleed vulnerability in OpenSSL exposed in 2014 has affected billions of Internet users \cite{Heartbleed}. Cyberattacks are constant threats to businesses, governments and consumers. The rate and cost of a cyber breach is increasing rapidly with annual cost to the global economy from cybercrime being estimated at \$400 billion \cite{McAfee}. In 2017, it is estimated that the global security market is worth \$120 billion \cite{CybersecurityVentures}. Central to security protection is the ability to detect and mitigate software vulnerabilities early, especially before software release to effectively prevent attackers from exploit them.

%exposed this problem: two missing lines of code compromised the integrity of a huge swathe of Internet infrastructure in 2014
%The global cyber and physical security industries are about \$80 billion. security incidents are growing at a compound annual growth rate of 66\% . Most cyberattacks have limited impacts, but a successful attack on some components of critical infrastructure (CI) most of which is held by the private sector http://cybersecurityventures.com/cybersecurity-market-report/

%\point{why predicting software components is useful. Help engineers to locate, etc. Problems with static tool analysis, high false positive. }

Software has significantly increased in both size and complexity. Identifying security vulnerabilities in software code is highly difficult since they are rare compared to other types of software defects. For example, the infamous Heartbleed vulnerability was caused only by two missing lines of code \cite{Heartbleed2014}. Finding software vulnerabilities is commonly referred to as ``searching for a needle in a haystack'' \cite{Zimmermann:2010:SNH}. Static analysis tools have been routinely used as part of the security testing process but they commonly generate a large number of false positives \cite{Austin:2011:OTE,Ceccato:2016:SAP}. Dynamic analysis tools rely on detailed monitoring of run-time properties including log files and memory, and require a wide range of representative test cases to exercise the application. Hence, standard practice still relies heavily on domain knowledge to identify the most vulnerable part of a software system for intensive security inspection.

Software engineers can be supported by automated tools that explore remaining parts of the code base more likely to contain vulnerabilities and raise an alert on these. Such predictive models and tools can help prioritize  effort and optimize inspection and testing costs. They aim to increase the likelihood of finding vulnerabilities and reduce the time required by software engineers to discover vulnerabilities. In addition, a predictive capability that identifies vulnerable components early in the software lifecycle is a significant achievement since the cost of finding and fixing errors increases dramatically as the software lifecycle progresses.

%\point{software metric features and its problem ....}

A common approach to build vulnerability prediction models is by using machine learning techniques. A number of features representing software code are selected for use as predictors for vulnerability. The most commonly used features in previous work (e.g. \cite{Shin:2011:ECC}) are software metrics (e.g. size of code, number of dependencies, and cyclomatic complexity), code churn metrics (e.g. the number of code lines changed), and developer activity. Those features cannot however distinguish code regions of different semantics and likelihood of vulnerability to attack. In many cases, two pieces of code may have the same complexity metrics but they behave differently. Furthermore, the choice of which features are selected as predictors is \emph{manually} are chosen by knowledgeable domain experts, and may thus cary outdated  experience and underlying biases. In addition, in many situations  handcrafted features normally do not generalize well:  features that work well in a  certain  software  project  may  not  perform  well  in  other projects \cite{Zimmermann:2009:CDP}.

An emerging approach is treating software code as a form of text and leveraging Natural Language Processing (NLP) techniques to automatically extract features. Previous work (e.g. \cite{ScandariatoWHJ14}) has used Bag-of-Words (BoW) to represent a source code file as a collection of code tokens associated with frequencies. The terms are the features which are used as the predictors for their vulnerability prediction model. Their set of features are thus fixed or pre-determined (as seen in the software metric model), but rather depend on the vocabulary used by developers. However, the BoW approach has two major weaknesses. Firstly,  it ignores the semantics of code tokens, e.g. fails to recognize the semantic relations between ``for'' and ``while''. Secondly, a bag of code tokens does not necessarily capture the semantic structure of code, especially its sequential nature.

%\input{sections/example}


%Coming up with good features which discriminate security vulnerabilities and other defects is however difficult and requires domain-specific knowledge.  .  In  addition,  handcrafted features often rely on expert knowledge, which  is  sometimes  based  on  outdated  experience  and  an underlying bias, thus impeding the discovery of new, useful features.

%\point{Our contribution: LSTM and multi instance learning ...}

The recent advances of deep learning models \cite{lecun2015deep} in machine learning offer a powerful alternative to software metrics and BoW in representing software code. The two most widely-used deep learning models are: (i) Long Short-Term Memory (LSTM) \cite{hochreiter1997long}, a special kind of recurrent neural networks that is highly effective in learning long-term dependencies in sequential data such as text and speech; and (ii) Convolutional Neural Networks (CNN) \cite{Cun:1990:HDR}, a deep feedforward neural network of multiple processing layers that is highly successful in learning representations of data with multiple levels of abstraction such as images and video.

This paper presents a novel deep learning-based model for predicting vulnerabilities in software code. Our prediction model leverages LSTM to capture the long context relationships in source code where dependent code elements are scattered far apart. For example, pairs of code tokens that are required to appear together due to programming language specification (e.g. $try$ and $catch$ in Java) or due to API usage specification (e.g. $lock()$ and $unlock()$), but do not immediately follow each other. We use LSTM to automatically learn (from a large number of valid code sequences) a vector representation for each method/function in a source code file. Unlike BoW, this representation sufficiently captures the semantics of code tokens as well the sequential structure of source code.

Our prediction model consists of multiple deep feedforward neural networks (one for each method/function in a source file and working like CNN) to detect code patterns within each method/function that are known to be useful for vulnerability detection. Our model is also able to discover interaction patterns between methods by allowing information exchanged between those neural networks. Overall, our model can \emph{automatically} discover the representations needed for detection or classification (e.g. vulnerability prediction) from raw data (e.g. code tokens), thereby removing the need for manual feature engineering which occupies most of the effort in traditional approaches (e.g. software metrics). Results from our experiments on 18 software apps for the Android OS platform from a public dataset \cite{ScandariatoWHJ14} demonstrate that our approach outperforms both the software metrics and the BoW approaches in predicting vulnerabilities in code.

%This code modeling component is part of our vision for DeepSoft \cite{DeepSoftFSE2016}, an \emph{end-to-end}, generic deep learning-based framework for modeling software and its development process.


%In this paper, we build a prediction model which can predict whether a source code file is likely to be vulnerable. This type of prediction is standard in the literature. The goal here is to alerts software engineers with parts of the code base that deserve particular attention, rather than pinpointing exactly the code line where a vulnerability is resided. We choose to work at the level of files since this is also the scope of existing work. To enable fair comparison, we also employ the same datasets used in previous work.

%We view each source file as a bag of instances where each instance is a method declaration, e.g. $doSomething()$ in the example if Figure \ref{fig:example}. In the datasets we used, each source file is labeled (as either vulnerable or not vulnerable) while there is no labelling on the methods. In other words, the labels are \emph{only} assigned to a bag of instances and there are no labels on each individual instance. The labelling was done under the assumption that a source file is marked as vulnerable if one or more of its methods are vulnerable. Here, we need to predict if a source file is vulnerable without knowing the vulnerability of its methods. To do so, we employ  multi-instance learning methods, which have been successful in drug activity prediction.


The outline of this paper is as follows. In the next section, we provide a brief background on vulnerability prediction and the neural networks used in our model. We then present our approach in Section 3 and report the experiments to evaluate it in Section 4. In Section 5, we discuss related work before summarizing the contributions of the paper and outlines future work in Section 6.








==> sections/old/related-work.tex <==
\section{Related work}


Machine learning techniques have been widely used to build vulnerability prediction models. Early approaches (e.g. \cite{Shin:2008:EMP}) employed complexity metrics such as (e.g. McCabe's  cyclomatic complexity, nesting complexity, and size) as the predictors. Later approaches enriched this software metric feature set with coupling and cohesion metrics (e.g. \cite{Chowdhury:2011:UCC}), code churn and developer activity metrics (e.g. \cite{Shin:2011:ECC})), and dependencies and organizational measures (e.g. \cite{Zimmermann:2010:SNH}). Those approaches require knowledgeable domain experts to determine the metrics that are used as predictors for vulnerability.

Recent approaches treat source code as another form of text and leverage text mining techniques to extract the features for building vulnerability prediction models. The work in \cite{ScandariatoWHJ14} used the Bag-of-Words representation in which a source code file is viewed as a set of terms with associated frequencies. They then used the term-frequencies as the features for predicting vulnerability. The BoW approach eliminates the need for manually designing the features. BoW models also produced higher recall than software metric models for PHP applications \cite{Walden:2014:PVC}. However, the BoW approaches carries the inherent limitation of BoW in which syntactic information such as code order is disregarded.

%The Effect of Dimensionality Reduction on Software Vulnerability Prediction Models

Predicting vulnerabilities is related to software defect prediction. The study in \cite{ShinW13} found that some defect prediction models can be adapted for vulnerability prediction. While code metrics were commonly used as features for building defect prediction models \cite{Hall:2012}, various other metrics have also been employed such as change-related metrics \cite{Moser:2008,Nagappan:2005:URC}, developer-related metrics \cite{Pinzger:2008:DNP}, organization metrics \cite{Nagappan:2008:IOS}, and change process metrics \cite{Hassan:2009:PFU}. Recently, a number of approaches (e.g. \cite{Yang:2015:DLJ,Wang:2016:ALS}) have leveraged a deep learning model called Deep Belief Network \cite{DBN-Hinton06} to automatically learn features for defect prediction.

Deep learning has recently attracted increasing interests in software engineering. The work in \cite{DeepSoftFSE2016} proposes generic deep learning framework based on LSTM for modeling software and its development process. The work in \cite{White:2015:TDL} demonstrated the effectiveness of using recurrent neural networks (RNN) to model source code over traditional approaches such as $n$-grams. Their later work \cite{White:2016:DLC} extended these RNN models for detecting code clones. The work in \cite{Gu:2016:DAL} uses a special RNN  Encoder--Decoder, which consists of an encoder RNN to process the input sequence and a  decoder  RNN  with  attention  to  generate  the  output  sequence, to generate  API  usage  sequences  for a  given  API-related  natural  language  query. The work in \cite{DBLP:conf/aaai/GuptaPKS17} also uses RNN Encoder--Decoder but for fixing common errors in C programs. The work \cite{DeepCode2016} showed that LSTM is even more effective in code modeling, which inspired us to use it for learning vulnerability features. The work in \cite{Huo:2016:LUF} uses CNN for bug localization. 



==> sections/old/results.tex <==

\subsection{Results}

\subsubsection{Learned code token semantics}

An important part of our approach is learning the semantics of code tokens using the context of its usage through LSTM. Figure \ref{figure:code-clusters} show the top 2,000 frequent code tokens used in our dataset. They were automatically grouped in 10 clusters (using K-means clustering) based on their token states learned through LSTM. Recall that these clusters are the basis for us to construct a codebook (discussed in Section \ref{subsec:codebook}). We used t-distributed stochastic neighbor embedding (t-SNE) \cite{van2008visualizing} to display high-dimensional vectors in two dimensions. Principle Component Analysis (PCA) is an alternative but PCA is generally poor in visualizing this kind of data due to its global properties at the document level. We show here some representative code tokens from some clusters for a brief illustration. Code tokens that are semantically related are grouped in the same cluster. For example, code tokens related to exceptions such as IllegalArgumentException, FileNotFoundException, and NoSuchMethodException are grouped in one cluster. This indicates, to some extent, that the learned token states effectively capture the semantic relations between code tokens, which is useful for us to learn both syntactic and semantic features later.

\begin{figure}[ht]
	\centering
	\includegraphics[width=\linewidth]{figs/10_clusters.pdf}
	\caption{Top 2,000 frequent code tokens were automatically grouped into clusters (each cluster has a distinct colors)}
	\label{figure:code-clusters}
\end{figure}


\subsubsection{Within-project prediction (RQ1)}

\begin{table*}[h]
\centering \caption{Within-version results (RQ1)}
\label{table:dataset-RQ1} \resizebox{7.0in}{!}{%
\begin{tabular}{@{}lcccccc@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\toprule
\multirow{2}{*}{App} & \multicolumn{3}{c}{Metrics} & \multicolumn{3}{c}{BoW} & \multicolumn{3}{c}{DBN} & \multicolumn{3}{c}{LSTM-M} & \multicolumn{3}{c}{LSTM-S} & \multicolumn{3}{c}{Codebook} & \multicolumn{3}{c}{Joint}\tabularnewline
 & \quad{}P \quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{}\tabularnewline
\midrule
AnkiAndroid  & 0.62 & 0.65 & 0.61 & 1.00 & 0.94 & 0.96 & 1.00 & 0.94 & 0.96 &  &  & 0.96 &  &  & 1.00 &  &  & 0.96 &  &  & 0.96\tabularnewline
Boardgamegeek  & 0.18 & 0.35 & 0.23 & 0.95 & 1.00 & 0.97 & 0.95 & 1.00 & 0.97 &  &  & 0.88 &  &  & 0.93 &  &  & 0.90 &  &  & 0.90\tabularnewline
Browser  & 0.65 & 0.60 & 0.62 & 0.96 & 1.00 & 0.98 & 0.96 & 1.00 & 0.98 &  &  & 0.98 &  &  & 1.00 &  &  & 0.98 &  &  & 0.98\tabularnewline
Calendar  & 0.52 & 0.43 & 0.45 & 0.89 & 0.80 & 0.83 & 1.00 & 0.91 & 0.94 &  &  & 0.96 &  &  & 1.00 &  &  & 0.94 &  &  & 1.00\tabularnewline
Camera  & 0.72 & 0.81 & 0.73 & 0.82 & 0.92 & 0.86 & 0.83 & 0.93 & 0.87 &  &  & 0.90 &  &  & 0.93 &  &  & 0.94 &  &  & 0.94\tabularnewline
Connectbot  & 0.65 & 0.73 & 0.64 & 0.97 & 0.90 & 0.91 & 0.92 & 0.90 & 0.88 &  &  & 0.97 &  &  & 0.98 &  &  & 0.93 &  &  & 0.93\tabularnewline
Contacts  & 0.72 & 0.72 & 0.71 & 0.94 & 0.88 & 0.89 & 0.92 & 0.81 & 0.83 &  &  & 0.89 &  &  & 0.95 &  &  & 0.89 &  &  & 0.90\tabularnewline
Coolreader  & 0.55 & 0.70 & 0.60 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 &  &  & 1.00 &  &  & 0.96 &  &  & 0.96 &  &  & 0.96\tabularnewline
Crosswords  & 0.55 & 0.57 & 0.55 & 0.89 & 0.89 & 0.89 & 0.89 & 0.89 & 0.89 &  &  & 0.85 &  &  & 0.89 &  &  & 0.85 &  &  & 0.85\tabularnewline
Deskclock  & 0.30 & 0.20 & 0.23 & 0.92 & 0.92 & 0.89 & 0.83 & 0.92 & 0.83 &  &  & 0.94 &  &  & 1.00 &  &  & 0.94 &  &  & 0.94\tabularnewline
Email  & 0.83 & 0.84 & 0.82 & 0.92 & 0.93 & 0.92 & 0.96 & 0.94 & 0.94 &  &  & 0.92 &  &  & 0.93 &  &  & 0.92 &  &  & 0.93\tabularnewline
Fbreader  & 0.60 & 0.52 & 0.55 & 0.78 & 0.88 & 0.81 & 0.81 & 0.85 & 0.82 &  &  & 0.85 &  &  & 0.82 &  &  & 0.84 &  &  & 0.83\tabularnewline
Gallery2  & 0.62 & 0.60 & 0.57 & 0.80 & 0.91 & 0.84 & 0.75 & 0.87 & 0.78 &  &  & 0.80 &  &  & 0.84 &  &  & 0.84 &  &  & 0.83\tabularnewline
K9  & 0.73 & 0.82 & 0.76 & 0.94 & 0.88 & 0.89 & 0.96 & 0.87 & 0.90 &  &  & 0.93 &  &  & 0.94 &  &  & 0.91 &  &  & 0.92\tabularnewline
Keepassdroid  & 0.69 & 0.75 & 0.71 & 0.91 & 0.88 & 0.88 & 0.85 & 0.90 & 0.87 &  &  & 0.93 &  &  & 0.94 &  &  & 0.89 &  &  & 0.88\tabularnewline
Mms  & 0.78 & 0.60 & 0.67 & 0.86 & 0.85 & 0.85 & 0.84 & 0.85 & 0.84 &  &  & 0.83 &  &  & 0.85 &  &  & 0.87 &  &  & 0.89\tabularnewline
Mustard  & 0.81 & 0.68 & 0.72 & 0.94 & 0.93 & 0.93 & 0.94 & 0.87 & 0.89 &  &  & 0.96 &  &  & 0.97 &  &  & 0.94 &  &  & 0.96\tabularnewline
Quicksearchbox  & 0.60 & 0.42 & 0.43 & 0.84 & 0.90 & 0.83 & 0.83 & 0.90 & 0.84 &  &  & 0.89 &  &  & 0.88 &  &  & 0.82 &  &  & 0.82\tabularnewline
\midrule
Average  & 0.62 & 0.61 & 0.59 & 0.91 & 0.91 & 0.90 & 0.90 & 0.91 & 0.89 &  &  & \textbf{0.91} &  &  & \textbf{0.93} &  &  & \textbf{0.91} &  &  & \textbf{0.91}\tabularnewline
\bottomrule
\end{tabular}}
\end{table*}


\subsubsection{Cross-version prediction (RQ2)}

\begin{table*}[h]
\centering \caption{Cross-version results (RQ2)}
\label{table:dataset-RQ2} \resizebox{7.0in}{!}{%
\begin{tabular}{@{}lcccccc@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\toprule
\multirow{2}{*}{App} & \multicolumn{3}{c}{Metrics} & \multicolumn{3}{c}{BoW} & \multicolumn{3}{c}{DBN} & \multicolumn{3}{c}{LSTM-M} & \multicolumn{3}{c}{LSTM-S} & \multicolumn{3}{c}{Codebook} & \multicolumn{3}{c}{Joint (bmm)}\tabularnewline
 & \quad{}P \quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & F\quad{} & \quad{}P\quad{} & \quad{}R\quad{} & \quad{}F\quad{}\tabularnewline
\midrule
AnkiAndroid  & 0.80 & 0.71 & 0.75 &  &  & 0.87 &  &  & 0.86 &  &  & 0.87 &  &  & 0.87 &  &  & 0.87 &  &  & 0.88\tabularnewline
Browser  & 0.69 & 0.65 & 0.66 &  &  & 0.68 &  &  & 0.70 &  &  & 0.65 &  &  & 0.61 &  &  & 0.68 &  &  & 0.68\tabularnewline
Calendar  & 0.69 & 0.77 & 0.72 &  &  & 0.78 &  &  & 0.78 &  &  & 0.78 &  &  & 0.77 &  &  & 0.83 &  &  & 0.82\tabularnewline
Camera  & 0.51 & 0.81 & 0.62 &  &  & 0.72 &  &  & 0.70 &  &  & 0.72 &  &  & 0.73 &  &  & 0.76 &  &  & 0.82\tabularnewline
Connectbot  & 0.75 & 0.75 & 0.75 &  &  & 0.98 &  &  & 0.98 &  &  & 1.00 &  &  & 1.00 &  &  & 1.00 &  &  & 1.00\tabularnewline
Contacts  & 0.68 & 0.72 & 0.70 &  &  & 0.73 &  &  & 0.74 &  &  & 0.66 &  &  & 0.69 &  &  & 0.70 &  &  & 0.71\tabularnewline
Coolreader  & 0.80 & 0.77 & 0.78 &  &  & 0.85 &  &  & 0.83 &  &  & 0.88 &  &  & 0.91 &  &  & 0.87 &  &  & 0.89\tabularnewline
Crosswords  & 0.87 & 0.72 & 0.79 &  &  & 0.86 &  &  & 0.85 &  &  & 0.87 &  &  & 0.87 &  &  & 0.89 &  &  & 0.87\tabularnewline
Deskclock  & 0.87 & 0.66 & 0.75 &  &  & 0.85 &  &  & 0.81 &  &  & 0.88 &  &  & 0.86 &  &  & 0.88 &  &  & 0.86\tabularnewline
Email  & 0.74 & 0.83 & 0.78 &  &  & 0.82 &  &  & 0.82 &  &  & 0.85 &  &  & 0.84 &  &  & 0.87 &  &  & 0.86\tabularnewline
Fbreader  & 0.83 & 0.75 & 0.78 &  &  & 0.81 &  &  & 0.77 &  &  & 0.82 &  &  & 0.83 &  &  & 0.88 &  &  & 0.85\tabularnewline
Gallery2  & 0.74 & 0.74 & 0.74 &  &  & 0.95 &  &  & 0.88 &  &  & 0.95 &  &  & 0.96 &  &  & 0.97 &  &  & 0.97\tabularnewline
K9  & 0.77 & 0.89 & 0.82 &  &  & 0.84 &  &  & 0.85 &  &  & 0.86 &  &  & 0.87 &  &  & 0.90 &  &  & 0.90\tabularnewline
Keepassdroid  & 0.92 & 0.91 & 0.91 &  &  & 0.89 &  &  & 0.86 &  &  & 0.98 &  &  & 0.99 &  &  & 0.94 &  &  & 0.95\tabularnewline
Mms  & 0.83 & 0.81 & 0.82 &  &  & 0.91 &  &  & 0.90 &  &  & 0.91 &  &  & 0.91 &  &  & 0.93 &  &  & 0.94\tabularnewline
Mustard  & 0.93 & 0.90 & 0.91 &  &  & 0.96 &  &  & 0.93 &  &  & 0.98 &  &  & 0.98 &  &  & 0.97 &  &  & 0.97\tabularnewline
Quicksearchbox  & 0.57 & 0.69 & 0.62 &  &  & 0.72 &  &  & 0.66 &  &  & 0.80 &  &  & 0.78 &  &  & 0.80 &  &  & 0.82\tabularnewline
\midrule
Average  & 0.76 & 0.77 & 0.76 &  &  & \textbf{0.84} &  &  & \textbf{ 0.82} &  &  & \textbf{ 0.85 } &  &  & \textbf{0.85} &  &  & \textbf{0.87} &  &  & \textbf{0.87}\tabularnewline
\bottomrule
\end{tabular}}
\end{table*}


\subsubsection{Cross-project prediction (RQ3)}

\begin{table*}[h]
\centering \caption{Cross-project results (RQ3)}
\label{table:dataset-stats-RQ3} \resizebox{6in}{!}{%
\begin{tabular}{lccccccc}
\toprule
App & Metrics  & BoW & DBN & LSTM-M & LSTM-S & Codebook
 & Joint (bmm)\tabularnewline
\midrule
AnkiAndroid  & 1  & 2 & 2 & 2 & 3 & 7 & 5\tabularnewline
Boardgamegeek  & 0  & 1 & 1 & 0 & 0 & 1 & 1\tabularnewline
Browser  & 0  & 1 & 2 & 2 & 0 & 0 & 1\tabularnewline
Calendar  & 0  & 1 & 1 & 1 & 1 & 4 & 5\tabularnewline
Camera  & 1  & 3 & 2 & 3 & 3 & 6 & 6\tabularnewline
Connectbot  & 0  & 2 & 2 & 4 & 4 & 4 & 5\tabularnewline
Contacts  & 0  & 1 & 3 & 2 & 1 & 2 & 2\tabularnewline
Coolreader  & 1  & 2 & 3 & 3 & 4 & 4 & 6\tabularnewline
Crosswords  & 0  & 3 & 3 & 2 & 2 & 1 & 1\tabularnewline
Deskclock  & 0  & 1 & 1 & 0 & 0 & 1 & 1\tabularnewline
Email  & 1  & 2 & 2 & 3 & 4 & 4 & 4\tabularnewline
Fbreader  & 0  & 2 & 2 & 3 & 4 & 6 & 6\tabularnewline
Gallery2  & 0  & 3 & 2 & 2 & 3 & 3 & 2\tabularnewline
K9  & 1  & 3 & 3 & 2 & 2 & 7 & 8\tabularnewline
Keepassdroid  & 0  & 3 & 1 & 3 & 4 & 2 & 4\tabularnewline
Mms  & 0  & 4 & 2 & 3 & 3 & 5 & 6\tabularnewline
Mustard  & 0  & 3 & 3 & 3 & 3 & 8 & 8\tabularnewline
Quicksearchbox  & 0  & 2 & 2 & 2 & 1 & 3 & 3\tabularnewline
\midrule
Average & 0.3 & 2.2 & 2.1 & 2.2 & 2.3 & 3.8 & 4.1\tabularnewline
Total & 5 &  39  &  37  & \textbf{ 40} & \textbf{42} & \textbf{ 68} & \textbf{ 74 }\tabularnewline
\bottomrule
\end{tabular}}
\end{table*}


==> sections/old/threats.tex <==
\section{Threats to validity}

There are a number of threats to the validity of our study, which we discuss below.


\textbf{Construct validity:} We mitigated the construct validity concerns by using a publicly available dataset that has been used in previous work \cite{ScandariatoWHJ14}. The dataset contains real Android applications and vulnerability labels of the files in those applications. The original dataset did not unfortunately contain the source files. However, we have carefully used the information (e.g. application details, version numbers and date) provided with the dataset to retrieve the relevant source files from the code repository of those applications. 


\textbf{Conclusion validity:} We tried to minimize threats to conclusion validity by using standard performance measures for vulnerability prediction \cite{ScandariatoWHJ14,Walden:2014:PVC,Shin:2011:ECC,Chowdhury:2011:UCC}. We however acknowledge that a number of statistical tests \cite{STVR:STVR1486} can be applied to verify the statistical significance of our conclusions. Although we have not seen those statistical tests being used in previous work in vulnerability prediction, we plan to do this investigation in our future work. 

	
\textbf{Internal validity:} The dataset we used contains vulnerability labels only for Java source files. In practice, other files (e.g. XML manifest files) may contain security information such as access rights. Another threat concerns the cross-version prediction where we replicated the experiment done in \cite{ScandariatoWHJ14} and allowed that the exactly same files might be present between versions. This might have inflated the results, but all the prediction models which we compared against in our experiment benefit from this. 


\textbf{External validity:} We have considered a large number of applications which differ significantly in size, complexity, domain, popularity and revision history. We however acknowledge that our data set may not be representative of all kinds of Android applications. Further investigation to confirm our findings for other Android applications as well as other types of applications such as web applications and applications written in other programming languages such as PhP and C++. 



==> sections/results-include-syn-features-m.tex <==

\subsection{Results}

\subsubsection{Learned code token semantics}

An important part of our approach is learning the semantics of code tokens using the context of its usage through LSTM. Figure \ref{figure:code-clusters} show the top 2,000 frequent code tokens used in our dataset. They were automatically grouped in 10 clusters (using K-means clustering) based on their token states learned through LSTM. Recall that these clusters are the basis for us to construct a codebook (discussed in Section \ref{subsec:codebook}). We used t-distributed stochastic neighbor embedding (t-SNE) \cite{van2008visualizing} to display high-dimensional vectors in two dimensions. Principle Component Analysis (PCA) is an alternative but PCA is generally poor in visualizing this kind of data due to its global properties at the document level. We show here some representative code tokens from some clusters for a brief illustration. Code tokens that are semantically related are grouped in the same cluster. For example, code tokens related to exceptions such as IllegalArgumentException, FileNotFoundException, and NoSuchMethodException are grouped in one cluster. This indicates, to some extent, that the learned token states effectively capture the semantic relations between code tokens, which is useful for us to learn both syntactic and semantic features later.

\begin{figure}[ht]
	\centering
	\includegraphics[width=\linewidth]{figs/10_clusters.pdf}
	\caption{Top 2,000 frequent code tokens were automatically grouped into clusters (each cluster has a distinct color)}
	\label{figure:code-clusters}
\end{figure}


\subsubsection{Within-project prediction (RQ1)}

We experimented with a number of variations of our approach by varying the pooling methods and the use of syntactic and semantic features. Table \ref{table:results-RQ1} reports the precision, recall and F-measure for the three benchmarks (software metrics, Bag-of-Words, and Deep Belief Network) and

Specifically, we are interested in four variations: using



\begin{table*}[ht]
\centering \caption{Within-projects results (RQ1) for the three benchmarks and four variations of our approach}
\label{table:results-RQ1} \resizebox{7.0in}{!}{%
%\begin{tabular}{@{}lcccccc@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\begin{tabular}{@{}l|ccc|ccc|ccc|ccc|ccc|ccc|ccc}
\toprule
\multirow{2}{*}{Application} & \multicolumn{3}{c}{Software metrics} & \multicolumn{3}{c}{Bag-of-Words} & \multicolumn{3}{c}{Deep Belief Network} & \multicolumn{3}{c}{\textbf{Syntactic features (M)}} & \multicolumn{3}{c}{\textbf{Syntactic features (S)}} & \multicolumn{3}{c}{\textbf{Semantic features}} & \multicolumn{3}{c}{\textbf{Joint features (SMS)}}\tabularnewline
 & {}P {} & {}R{} & {}F{} & {}P{} & {}R{} & {}F{} & {}P{} & {}R{} & {}F{} & {}P{} & {}R{} & {}F{} & {}P{} & {}R{} & {}F{} & {}P{} & {}R{} & F{} & {}P{} & {}R{} & {}F{}\tabularnewline
\midrule
AnkiAndroid  & 0.62 & 0.65 & 0.61 & 1.00 & 0.94 & 0.96 & 1.00 & 0.94 & 0.96 & 1.00 & 0.94 & 0.96 & 1.00 & 1.00 & 1.00 & 1.00 & 0.94  & 0.96 & 1.00 & 0.94 & 0.96\tabularnewline
Boardgamegeek  & 0.18 & 0.35 & 0.23 & 0.95 & 1.00 & 0.97 & 0.95 & 1.00 & 0.97 & 0.87 & 0.90 & 0.88 & 0.95 & 0.95 & 0.93 & 0.90 & 0.90 & 0.90 & 0.90 & 0.90 & 0.90\tabularnewline
Browser  & 0.65 & 0.60 & 0.62 & 0.96 & 1.00 & 0.98 & 0.96 & 1.00 & 0.98 & 0.96 & 1.00 & 0.98 & 1.00  & 1.00 & 1.00 & 0.96 & 1.00 & 0.98 & 0.96 & 1.00 & 0.98\tabularnewline
Calendar  & 0.52 & 0.43 & 0.45 & 0.89 & 0.80 & 0.83 & 1.00 & 0.91 & 0.94 & 0.96 & 0.96 & 0.96 & 1.00  & 1.00 & 1.00 & 0.96 & 0.94 & 0.94 & 1.00 & 1.00 & 1.00\tabularnewline
Camera  & 0.72 & 0.81 & 0.73 & 0.82 & 0.92 & 0.86 & 0.83 & 0.93 & 0.87 & 0.85 & 1.00  & 0.90 & 0.88  & 1.00 & 0.93 & 0.92 & 0.98 & 0.94 & 0.92 & 0.98 & 0.94\tabularnewline
Connectbot  & 0.65 & 0.73 & 0.64 & 0.97 & 0.90 & 0.91 & 0.92 & 0.90 & 0.88 & 1.00 & 0.94 & 0.97 & 1.00 & 0.97 & 0.98 & 0.93 & 0.93 & 0.93 & 0.97 & 0.93 & 0.93\tabularnewline
Contacts  & 0.72 & 0.72 & 0.71 & 0.94 & 0.88 & 0.89 & 0.92 & 0.81 & 0.83 & 0.90 & 0.92  & 0.89 & 0.96  & 0.94 & 0.95 & 0.89  & 0.94 & 0.89 & 0.87 & 0.97 & 0.90\tabularnewline
Coolreader  & 0.55 & 0.70 & 0.60 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 0.94 & 0.96 & 1.00 & 0.94 & 0.96 & 1.00 & 0.94 & 0.96\tabularnewline
Crosswords  & 0.55 & 0.57 & 0.55 & 0.89 & 0.89 & 0.89 & 0.89 & 0.89 & 0.89 & 0.89 & 0.83 & 0.85 & 0.89 & 0.89 & 0.89 & 0.89 & 0.83 & 0.85 & 0.89 & 0.83 & 0.85\tabularnewline
Deskclock  & 0.30 & 0.20 & 0.23 & 0.92 & 0.92 & 0.89 & 0.83 & 0.92 & 0.83 & 0.92 & 1.00 & 0.94 & 1.00 & 1.00  & 1.00 & 1.00 & 0.92 & 0.94 & 1.00 & 0.92 & 0.94\tabularnewline
Email  & 0.83 & 0.84 & 0.82 & 0.92 & 0.93 & 0.92 & 0.96 & 0.94 & 0.94 & 0.93 & 0.92 & 0.92 & 0.93 & 0.95 & 0.93 & 0.95 & 0.90 & 0.92 & 0.94 & 0.93 & 0.93\tabularnewline
Fbreader  & 0.60 & 0.52 & 0.55 & 0.78 & 0.88 & 0.81 & 0.81 & 0.85 & 0.82 & 0.89 & 0.83 & 0.85 & 0.83 & 0.82 & 0.82 & 0.85 & 0.83 & 0.84 & 0.82 & 0.86 & 0.83\tabularnewline
Gallery2  & 0.62 & 0.60 & 0.57 & 0.80 & 0.91 & 0.84 & 0.75 & 0.87 & 0.78 & 0.79 & 0.84 & 0.80 & 0.83 & 0.88 & 0.84 & 0.83 & 0.87 & 0.84 & 0.80 & 0.89 & 0.83\tabularnewline
K9  & 0.73 & 0.82 & 0.76 & 0.94 & 0.88 & 0.89 & 0.96 & 0.87 & 0.90 & 0.91 & 0.96 & 0.93 & 0.89 & 1.00 & 0.94 & 0.88 & 0.97 & 0.91 & 0.88 & 0.98 & 0.92\tabularnewline
Keepassdroid  & 0.69 & 0.75 & 0.71 & 0.91 & 0.88 & 0.88 & 0.85 & 0.90 & 0.87 & 0.90 & 0.97 & 0.93 & 0.93 & 0.97 & 0.94 & 0.90 & 0.91 & 0.89 & 0.88 & 0.89 & 0.88\tabularnewline
Mms  & 0.78 & 0.60 & 0.67 & 0.86 & 0.85 & 0.85 & 0.84 & 0.85 & 0.84 & 0.81 & 0.88 & 0.83 & 0.87 & 0.85 & 0.85 & 0.87 & 0.88 & 0.87 & 0.87 & 0.92 & 0.89\tabularnewline
Mustard  & 0.81 & 0.68 & 0.72 & 0.94 & 0.93 & 0.93 & 0.94 & 0.87 & 0.89 & 0.95 & 0.98 & 0.96 & 0.96 & 0.99 & 0.97 & 0.97 & 0.93 & 0.94 & 0.95 & 0.99 & 0.96\tabularnewline
Quicksearchbox  & 0.60 & 0.42 & 0.43 & 0.84 & 0.90 & 0.83 & 0.83 & 0.90 & 0.84 & 0.94 & 0.89 & 0.89 & 0.93 & 0.90 & 0.88 & 0.89 & 0.77 & 0.82 & 0.89 & 0.79 & 0.82\tabularnewline
\midrule
Average  & 0.62 & 0.61 & 0.59 & 0.91 & 0.91 & 0.90 & 0.90 & 0.91 & 0.89 & \textbf{ 0.92} & \textbf{0.93} & \textbf{0.91} & \textbf{0.94} & \textbf{0.95} & \textbf{0.93} & \textbf{0.92} & \textbf{ 0.91} & \textbf{0.91} & \textbf{0.92} & \textbf{ 0.93} & \textbf{0.91}\tabularnewline
\bottomrule
\end{tabular}}
\end{table*}


\subsubsection{Cross-version prediction (RQ2)}

\begin{table*}[ht]
\centering \caption{Cross-version results (RQ2)}
\label{table:dataset-RQ2} \resizebox{7.0in}{!}{%
%\begin{tabular}{@{}lcccccc@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}c@{}}
\begin{tabular}{@{}lccccccccccccccccccccc}
\toprule
\multirow{2}{*}{Application} & \multicolumn{3}{c}{Software metrics} & \multicolumn{3}{c}{Bag-of-Words} & \multicolumn{3}{c}{Deep Belief Network} & \multicolumn{3}{c}{\textbf{LSTM-M}} & \multicolumn{3}{c}{\textbf{LSTM-S}} & \multicolumn{3}{c}{\textbf{Codebook}} & \multicolumn{3}{c}{\textbf{Joint (bmm)}}\tabularnewline
 & {}P {} & {}R{} & {}F{} & {}P{} & {}R{} & {}F{} & {}P{} & {}R{} & {}F{} & {}P{} & {}R{} & {}F{} & {}P{} & {}R{} & {}F{} & {}P{} & {}R{} & F{} & {}P{} & {}R{} & {}F{}\tabularnewline
\midrule
AnkiAndroid  & 0.80 & 0.71 & 0.75 & 0.88 & 0.85 & 0.87 & 0.87 & 0.85 & 0.86 & 0.93 & 0.82 & 0.87 & 0.83 & 0.90 & 0.87 & 0.91 & 0.84 & 0.87 & 0.89 & 0.87 & 0.88\tabularnewline
Browser  & 0.69 & 0.65 & 0.66 & 0.75 & 0.63 & 0.68 & 0.75 & 0.65 & 0.70 & 0.73 & 0.59 & 0.65 & 0.59 & 0.64 & 0.61 & 0.84 & 0.57 & 0.68 & 0.82 & 0.58 & 0.68\tabularnewline
Calendar  & 0.69 & 0.77 & 0.72 & 0.74 & 0.83 & 0.78 & 0.71 & 0.85 & 0.78 & 0.75 & 0.81 & 0.78 & 0.73 & 0.81 & 0.77 & 0.79 & 0.89 & 0.83 & 0.79 & 0.84 & 0.82\tabularnewline
Camera  & 0.51 & 0.81 & 0.62 & 0.60 & 0.90 & 0.72 & 0.58 & 0.89 & 0.70 & 0.66 & 0.79 & 0.72 & 0.65 & 0.84 & 0.73 & 0.67 & 0.88 & 0.76 & 0.84 & 0.80 & 0.82\tabularnewline
Connectbot  & 0.75 & 0.75 & 0.75 & 1.00 & 0.96 & 0.98 & 1.00 & 0.96 & 0.98 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00 & 1.00\tabularnewline
Contacts  & 0.68 & 0.72 & 0.70 & 0.74 & 0.71 & 0.73 & 0.73 & 0.75 & 0.74 & 0.65 & 0.66 & 0.66 & 0.60 & 0.80 & 0.69 & 0.69 & 0.72 & 0.70 & 0.73 & 0.69 & 0.71\tabularnewline
Coolreader  & 0.80 & 0.77 & 0.78 & 0.93 & 0.79 & 0.85 & 0.83 & 0.82 & 0.83 & 0.89 & 0.88 & 0.88 & 0.94 & 0.89 & 0.91 & 0.89 & 0.85 & 0.87 & 0.92 & 0.86 & 0.89\tabularnewline
Crosswords  & 0.87 & 0.72 & 0.79 & 0.90 & 0.81 & 0.86 & 0.83 & 0.88 & 0.85 & 0.90  & 0.84 & 0.87 & 0.85 & 0.89 & 0.87 & 0.88 & 0.90 & 0.89 & 0.92 & 0.83 & 0.87\tabularnewline
Deskclock  & 0.87 & 0.66 & 0.75 & 0.89 & 0.80 & 0.85 & 0.87 & 0.76  & 0.81 & 0.90 & 0.86 & 0.88 & 0.93 & 0.80 & 0.86 & 0.90 & 0.86 & 0.88 & 0.89 & 0.82 & 0.86\tabularnewline
Email  & 0.74 & 0.83 & 0.78 & 0.82 & 0.83 & 0.82 & 0.79 & 0.85 & 0.82 & 0.79 & 0.93 & 0.85 & 0.77 & 0.93 & 0.84 & 0.86 & 0.89 & 0.87 & 0.83 & 0.90 & 0.86\tabularnewline
Fbreader  & 0.83 & 0.75 & 0.78 & 0.79 & 0.83 & 0.81 & 0.80 & 0.75 & 0.77 & 0.88 & 0.77 & 0.82 & 0.84 & 0.81 & 0.83 & 0.91 & 0.84 & 0.88 & 0.86 & 0.84 & 0.85\tabularnewline
Gallery2  & 0.74 & 0.74 & 0.74 & 0.96 & 0.93 & 0.95 & 0.88 & 0.88 & 0.88 & 0.94 & 0.97 & 0.95 & 0.95 & 0.97 & 0.96 & 0.96 & 0.99 & 0.97 & 0.96 & 0.97 & 0.97\tabularnewline
K9  & 0.77 & 0.89 & 0.82 & 0.85 & 0.84 & 0.84 & 0.84 & 0.86 & 0.85 & 0.83 & 0.89 & 0.86 & 0.80 & 0.94 & 0.87 & 0.84 & 0.98 & 0.90 & 0.89 & 0.92 & 0.90\tabularnewline
Keepassdroid  & 0.92 & 0.91 & 0.91 & 0.92 & 0.87 & 0.89 & 0.86 & 0.86 & 0.86 & 0.99 & 0.97 & 0.98 & 1.00  & 0.99 & 0.99 & 0.98 & 0.91 & 0.94 & 0.99 & 0.92 & 0.95\tabularnewline
Mms  & 0.83 & 0.81 & 0.82 & 0.93 & 0.90 & 0.91 & 0.94 & 0.86 & 0.90 & 0.94 & 0.89 & 0.91 & 0.93 & 0.89 & 0.91 & 0.93 & 0.93 & 0.93 & 0.92 & 0.96 & 0.94\tabularnewline
Mustard  & 0.93 & 0.90 & 0.91 & 0.97 & 0.96 & 0.96 & 0.92 & 0.93 & 0.93 & 0.99 & 0.98 & 0.98 & 0.98 & 0.98 & 0.98 & 0.99 & 0.95 & 0.97 & 0.99 & 0.95 & 0.97\tabularnewline
Quicksearchbox  & 0.57 & 0.69 & 0.62 & 0.71 & 0.73 & 0.72 & 0.56 & 0.79 & 0.66 & 0.83 & 0.78 & 0.80 & 0.76 & 0.80 & 0.78 & 0.74 & 0.87 & 0.80 & 0.77 & 0.88 & 0.82\tabularnewline
\midrule
Average  & 0.76 & 0.77 & 0.76 & 0.85 & 0.83 & 0.84 & 0.81 &  0.84 & \textbf{ }0.82 & 0.86 &  0.85 & \textbf{ 0.85 } & 0.83 & 0.87 & \textbf{0.85} & 0.87 &  0.87 & \textbf{0.87} & 0.88 & 0.86 & \textbf{0.87}\tabularnewline
\bottomrule
\end{tabular}}
\end{table*}


\subsubsection{Cross-project prediction (RQ3)}

\begin{table*}[h]
\centering \caption{Cross-project results (RQ3)}
\label{table:dataset-stats-RQ3} \resizebox{6in}{!}{%
\begin{tabular}{lccccccc}
\toprule
Application & Software metrics  & Bag-of-Words & Deep Belief Network & \textbf{LSTM-M} & \textbf{LSTM-S} & \textbf{Codebook} & \textbf{Joint (bmm)}\tabularnewline
\midrule
AnkiAndroid  & 1  & 2 & 2 & 2 & 3 & 7 & 5\tabularnewline
Boardgamegeek  & 0  & 1 & 1 & 0 & 0 & 1 & 1\tabularnewline
Browser  & 0  & 1 & 2 & 2 & 0 & 0 & 1\tabularnewline
Calendar  & 0  & 1 & 1 & 1 & 1 & 4 & 5\tabularnewline
Camera  & 1  & 3 & 2 & 3 & 3 & 6 & 6\tabularnewline
Connectbot  & 0  & 2 & 2 & 4 & 4 & 4 & 5\tabularnewline
Contacts  & 0  & 1 & 3 & 2 & 1 & 2 & 2\tabularnewline
Coolreader  & 1  & 2 & 3 & 3 & 4 & 4 & 6\tabularnewline
Crosswords  & 0  & 3 & 3 & 2 & 2 & 1 & 1\tabularnewline
Deskclock  & 0  & 1 & 1 & 0 & 0 & 1 & 1\tabularnewline
Email  & 1  & 2 & 2 & 3 & 4 & 4 & 4\tabularnewline
Fbreader  & 0  & 2 & 2 & 3 & 4 & 6 & 6\tabularnewline
Gallery2  & 0  & 3 & 2 & 2 & 3 & 3 & 2\tabularnewline
K9  & 1  & 3 & 3 & 2 & 2 & 7 & 8\tabularnewline
Keepassdroid  & 0  & 3 & 1 & 3 & 4 & 2 & 4\tabularnewline
Mms  & 0  & 4 & 2 & 3 & 3 & 5 & 6\tabularnewline
Mustard  & 0  & 3 & 3 & 3 & 3 & 8 & 8\tabularnewline
Quicksearchbox  & 0  & 2 & 2 & 2 & 1 & 3 & 3\tabularnewline
\midrule
Average & 0.3 & 2.2 & 2.1 & 2.2 & 2.3 & 3.8 & 4.1\tabularnewline
Total & 5 &  39  &  37  & \textbf{ 40} & \textbf{42} & \textbf{ 68} & \textbf{ 74 }\tabularnewline
\bottomrule
\end{tabular}}
\end{table*}



